Koszulness and supersolvability for Dirichlet arrangements

We prove that the cone over a Dirichlet arrangement is supersolvable if and only if its Orlik-Solomon algebra is Koszul. This was previously shown for four other classes of arrangements. We exhibit an infinite family of cones over Dirichlet arrangements that are combinatorially distinct from these other four classes.

==> sections/falk.tex <==
\section{Falk invariants}
\label{sec:falk}

 Falk posed the problem of interpreting $\phi_3$ combinatorially \cite[Problem 1.4]{falk2001}. This problem was solved by Schenck and Suciu for graphic arrangements, and later by Guo, Guo, Hu and Jiang for arrangements associated to certain signed graphs.\todo{keep going! and cite} Guo and Torielli 

The Orlik-Solomon ideal $I$ inherits a grading $I^p$ from $F$. Let $I_q$ be the ideal of $F$ generated by $I^0 + I^1 + \cdots + I^q$. The ideal $I_q$ is called the \emph{$q$-adic closure} of $I$ and inherits a grading $I_q^p = (I_q)^p$ from $F$. The algebra $A_q = F/I_q$ is called the \emph{$q$-adic closure} of $A$ and also inherits a grading $A_q^p = (A_q)^p$ from $F$.

\begin{mydef}
	Consider the linear map $F^1\otimes I^2 \to F^3$ defined by $a\otimes b \mapsto ab$. The nullity of this map is denoted by $\phi_3$ and called the \emph{Falk invariant} of $L_0(N)$.
	\label{def:falk}
\end{mydef}

We say that $S\subset E$ is a \emph{short crossing} (resp., \emph{Wheatstone bridge}) if it induces the subgraph on the left (resp., right) side of Figure \ref{fig:scwb}, respecting the placement of the nodes and interior vertices. We say that $S\subset E$ is a \emph{triangle} (resp., a $K_4$) if it induces the complete subgraph $K_3$ (resp., $K_4$), with no distinction between nodes and interior vertices.

\begin{figure}[ht]
	\centering
	\input{tikz/falk1}
	\caption{Left to right: a short crossing and a Wheatstone bridge with nodes marked in white.}
	\label{fig:scwb}
\end{figure}

\begin{figure}[ht]
	\centering
	\input{tikz/falk2}
	\caption{The four types of generators (fix this).}
	\label{fig:4gens}
\end{figure}


\begin{thm}
	The Falk invariant of the Kirchhoff matroid $L_0(N)$ is given by
	\[\phi_3 = 2(\kap_1+\kap_2+\kap_3+\kap_4),\]
	where $\kap_1$ is the number of short crossings of $N$, $\kap_2$ is the number of Wheatstone bridges in $N$, $\kap_3$ is the number of triangles in $\g$, and $\kap_4$ is the number of $K_4$ in $\g$.
\end{thm}

\begin{remark}
	The notation $\phi_3$ for the Falk invariant comes from the topology of hyperplane arrangements. Let $\u:\B\to \R$ be injective, and let $\AA$ be the cone of the Kirchhoff arrangement associated to $(N,\u)$. Let $\pi$ be the fundamental group of the complement of the complexified arrangement $\C\otimes \AA$, and let $\pi=G_1,G_2,\ldots$ be the lower central series of $\pi$. Then every quotient $G_i/G_{i+1}$ is a finitely generated abelian group. Denoting the rank of $G_i/G_{i+1}$ by $\phi_i$ is consistent with Definition \ref{def:falk}.
\end{remark}

In this section write $k=|\eo|$.

\begin{prop}[{\cite[Theorem 4.7]{falk2001}}]
	The Falk invariant $\phi_3$ of $L_0(N)$ can be written in terms of $A$:
	\[\phi_3 = 2\binom{k+1}{3} - k \dim(A^2) + \dim(A^2_3).\]
\end{prop}

\begin{prop}
	We have
	\[\dim(A^2) = \binom{k}{2} - \kap_1 - \kap_3.\]
\end{prop}

Let $\triangle\subset \binom{E}{3}$ be the set of triangles in $\g$, and let $C\subset \binom{E}{2}$ be the set of short crossings of $N$. Define the following subsets of $F^3$:
\begin{align*}
S_\triangle &= \{ ijk : \{i,j,k\}\in \triangle\}\\
S_C &= \{ij\eh : \{i,j\}\in C\}\\
S_{W} &= \{t\dif (ijk) : t,i,j,k\mbox{ are illustrated in Figure \ref{fig:4gens}}\}\\
S_{K_4} &= \{t\dif(ijk) : \{i,j,k\}\in \triangle \mbox{ and } i,j,k,t\mbox{ belong to a }K_4\}\\
S_0 &= \{\eh \dif(ijk) :  \{i,j,k\}\in \triangle\}\setminus S_{W}\\
S_1 &= \{t\dif (ijk) : \{i,j,k\}\in \triangle\mbox{ and }t\in E\}\setminus (S_\triangle \cup S_{K_4} \cup S_0)\\
S_2 &= \{t\dif(ij\eh) : \{i,j\}\in C\} \setminus (S_C\cup S_W).
\end{align*}
For each $S_i$, let $U_i$ denote the span in $F^3$ of $S_i$.

\begin{lem}
	The vector space $I_3^2$ decomposes\todo{check these exp/sub} as
	\[I_3^2 = U_\triangle \oplus U_C \oplus U_W \oplus U_{K_4} \oplus U_0 \oplus U_1\oplus U_2.\]
\end{lem}

\begin{lem}
	Let $\mu$ be the number of triangles in $\g$ contained in Wheatstone bridges of $N$. We have
	\begin{align*}
	\dim U_\triangle &= \kap_3\\
	\dim U_C &= \kap_1\\
	\dim U_W &= 8\kap_2 + \mu\\
	\dim U_{K_4} &= 10\kap_4\\
	\dim U_0 &= \kap_3 - \mu\\
	\dim U_1 &= -4\kap_2 + (k-4)\kap_3 - 12\kap_4\\
	\dim U_2 &= (k-3)\kap_1-6\kap_2.
	\end{align*}
\end{lem}

\begin{prop}
	We have
	\[\dim(A_3^2) = \binom{k}{3} - (k-2)(\kap_1 + \kap_3) + 2(\kap_2 + \kap_4).\]
\end{prop}



==> sections/intro.tex <==
\section{Introduction}

Let $U$ be the complement of a central complex hyperplane arrangent $\AA$, and consider the lower central series $G_1,G_2,\ldots$ of the fundamental group $\pi_1(U)$. Some arrangements $\AA$ satisfy the celebrated \emph{Lower Central Series Formula}:
\begin{equation}
	\prod_{k=1}^\infty (1-t^k)^{\phi_k} = P(U,-t),
	\label{eq:lcsformula}
\end{equation}
where $\phi_k$ is the rank of $G_k/G_{k+1}$ and $P(U,t)$ is the Poincar\'{e} polynomial of $U$. In particular, \eqref{eq:lcsformula} is satisfied whenever the Orlik-Solomon algebra $\os(\AA)$ of $\AA$ is \emph{Koszul}, meaning that $\os(\AA)$ admits a certain kind of graded resolution. Thus it is natural to ask which arrangements have Koszul Orlik-Solomon algebras. Shelton and Yuzvinsky \cite[Theorem 4.6]{shelton1997} showed that if $\AA$ is supersolvable, then $\os(\AA)$ is Koszul. Whether the converse holds is unknown.

\begin{q}
	If the Orlik-Solomon algebra of a central hyperplane arrangement $\AA$ is Koszul, then is $\AA$ supersolvable?
	\label{q:koszul}
\end{q}

 Our main contribution is an affirmative answer for cones (or centralizations) over \emph{Kirchhoff arrangements}, a generalization of graphic arrangements arising from electrical networks and order polytopes of finite posets \cite{lutz2017,lutz2018mat}.

\begin{thm}
	The cone over a Kirchhoff arrangement is supersolvable if and only if its Orlik-Solomon algebra is Koszul.
	\label{thm:intro}
\end{thm}

Question \ref{q:koszul} has been answered affirmatively for certain other classes of arrangements, including graphic arrangements \cite{hultman2016,jambu1998, schenck2002, vanle2013}. To show that Theorem \ref{thm:intro} properly extends these results, we prove Theorem \ref{thm:intro2} below. We say that two central arrangements are \emph{combinatorially equivalent} if the underlying matroids are isomorphic.

\begin{thm}
	There are infinitely many cones over Kirchhoff arrangements that are not combinatorially equivalent to any arrangement for which Question \ref{q:koszul} has been previously answered.
	\label{thm:intro2}
\end{thm}

%In the appendix, we give a graph-theoretic formula for $\phi_3$, the \emph{Falk invariant} of the cone over a Kirchhoff arrangement, that is almost a special case of a result of Guo and Torielli \cite{guo2017}.
